Data-driven turbulence modeling

This chapter provides an introduction to data-driven techniques for the development and calibration of closure models for the Reynolds-Averaged Navier--Stokes (RANS) equations. RANS models are the workhorse for engineering applications of computational fluid dynamics (CFD) and are expected to play an important role for decades to come. However, RANS model inadequacies for complex, non-equilibrium flows and uncertainties in modeling assumptions and calibration data are still a major obstacle to the predictive capability of RANS simulations. In the following, we briefly recall the origin and limitations of RANS models, and then review their shortcomings and uncertainties. Then, we provide an introduction to data-driven approaches to RANS turbulence modeling. The latter can range from simple model parameter inference to sophisticated machine learning techniques. We conclude with some perspectives on current and future research trends.

==> header.tex <==
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{bm}
%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}
%% The amsthm package provides extended theorem environments
\usepackage{amsthm}
% \usepackage[titletoc]{appendix}
\usepackage[toc,page]{appendix}

% \usepackage{natbib}

%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers after \end{frontmatter}.
\usepackage{lineno}
\usepackage{subfig}
% \usepackage{enumerate}
\usepackage{fullpage}
%\usepackage{algorithm2e}
\usepackage{algorithm}
\usepackage{algpseudocode}
%\usepackage[monochrome]{xcolor}
\usepackage{array}
\usepackage{pbox}
\usepackage{tikz}
%
%\usepackage[final]{changes}
\usepackage[]{changes}
\usepackage[colorinlistoftodos]{todonotes}
%\usepackage[colorinlistoftodos,disable]{todonotes}

\def\onedot{$\mathsurround0pt\ldotp$}
\def\cddots{% two dots stacked vertically
  \mathbin{\vcenter{\baselineskip.67ex
    \hbox{\onedot}\hbox{\onedot}}%
  }}%

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% for inline annotation
\usepackage{url}
\usepackage{listings}
\usepackage[colorlinks=true]{hyperref}
\newtheorem{theorem}{Theorem}[]
\newtheorem{remark}{Remark}[]

\usepackage{color,soul}
\usepackage{mathtools}
\usepackage{booktabs}

\usepackage[colorlinks=true]{hyperref}

% For roadmap figure
\usepackage{forest}	
\usetikzlibrary{arrows.meta, shapes.geometric, calc, shadows}



% Added by Zeng Yang
\usepackage{multicol}
\usepackage{imakeidx}
\usepackage{nomencl}
\makenomenclature
\setlength{\nomitemsep}{-0.5\parsep}

\usepackage{etoolbox}
\renewcommand\nomgroup[1]{%
  \item[\itshape%\bfseries
  \ifstrequal{#1}{A}{Symbols}{%
  \ifstrequal{#1}{B}{Roman Letters}{%
  \ifstrequal{#1}{C}{Greek Letters}{%
  \ifstrequal{#1}{D}{Abbreviations}{}}}}%
]}
 
% This will add the units
%----------------------------------------------
\newcommand{\nomunit}[1]{%
\renewcommand{\nomentryend}{\hspace*{\fill}#1}}
%----------------------------------------------
\renewcommand{\nompreamble}{\begin{multicols}{2}}
\renewcommand{\nompostamble}{\end{multicols}}
% End of Zeng Yang contribution for nomenclature

% Collaboration tools
\definecolor{lightblue}{rgb}{.90,.95,1}
\definecolor{lightgreen}{rgb}{.90,1,.95}
\definecolor{darkgreen}{rgb}{0,.5,0.5}


% \usepackage{hyperref}
%% natbib.sty is loaded by default. However, natbib options can be
%% provided with \biboptions{...} command. Following options are
%% valid:

%\biboptions{sort,compress} 


% fixed line numbering
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}% 
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../mfu-main"
%%% End: 



==> nomenclature.tex <==
\nomenclature[A, 01]{$\overline{\boxed{\cdot}}$}{ensemble averaging or spatial filtering}
\nomenclature[A, 02]{$\lvert\lvert \cdot \rvert\rvert_{L^2}$ }{L2 norm}
\nomenclature[A, 03]{$\lvert\lvert A \rvert\rvert_{\mathsf{P}}$}{norm of $A$ weighted by covariance matrix $\mathsf{P}^{-1}$, i.e., $\lvert\lvert A^\top \mathsf{P}^{-1} A\rvert\rvert$}
\nomenclature[A, 04]{$\star$}{perturbed quantities}
\nomenclature[A, 05]{$\boxed{\cdot}^\top$}{transpose of vectors and matrices}
\nomenclature[A, 06]{$:$}{double dot of tensors $\tau_{ij} \frac{\partial U_i}{\partial x_j} \equiv \bm{\tau} \cddots \nabla \mathbf{U}$}
\nomenclature[A, 07]{$\circ$}{Hadamard (element-wise) multiplication}


\nomenclature[B, 01]{$\mathbf{a}$}{anisotropy tensor}
\nomenclature[B, 02]{$c_1$, $c_2$, $c_3$}{barycentric coordinates}
\nomenclature[B, 03]{$C_{\varepsilon1}$,$C_{\varepsilon2}$,$C_{\mu}$}{RANS model coefficients}
\nomenclature[B, 03b]{$C_{s}$}{Smagorinsky constant}
\nomenclature[B, 03c]{$\cov$}{covariance of random variables}
\nomenclature[B, 04]{$\bm{d}$}{discrepancy of observation and truth}
\nomenclature[B, 04]{$\frac{D \cdot}{D t}$}{material derivative}
\nomenclature[B, 05]{$\mathcal{D}$}{data used for inference}
\nomenclature[B, 05]{$D_\omega$}{dissipation of turbulent frequency}
\nomenclature[B, 06a]{$\mathbb{E}[Z]$}{expectation of random variable $Z$}
\nomenclature[B, 06b]{$f$}{functional mapping}
\nomenclature[B, 07]{$\mathcal{GP}(\cdot, \cdot)$}{Gaussian process}
\nomenclature[B, 08]{$\mathbf{h}$}{unit quaternion}
\nomenclature[B, 09a]{$\mathsf{H}$}{observation matrix}
\nomenclature[B, 09b]{$i, j, k$}{indices}
\nomenclature[B, 10]{$\mathbf{I}$}{second-order identity tensor}
\nomenclature[B, 10]{$I$}{number of scenarios}
\nomenclature[B, 11]{$J$}{objective function in optimization}
\nomenclature[B, 12]{$k$}{turbulent kinetic energy}
\nomenclature[B, 12]{$K(\cdot, \cdot)$}{kernel function of Gaussian process}
\nomenclature[B, 13]{$\mathsf{K}$}{Kalman gain matrix (in EnKF)}
\nomenclature[B, 13]{$K$}{number of models}
\nomenclature[B, 14a]{$l$}{length scale in covariance kernel}
\nomenclature[B, 14b]{$\mathcal{L}$}{linear differential operator}
\nomenclature[B, 15]{$\mathcal{M}$, $M_i$}{set of models; model}
\nomenclature[B, 16]{$\mathbf{n}$}{axis of rotation}
\nomenclature[B, 16]{$\mathsf{N}$}{normal distribution}
\nomenclature[B, 16b]{$\mathcal{N}$}{nonlinear differential operator}
\nomenclature[B, 17]{$\mathcal{O}(\cdot)$}{of the order of}
\nomenclature[B, 18]{$p$}{instantaneous pressure}
\nomenclature[B, 19]{$p'$ }{pressure fluctuation}
\nomenclature[B, 20]{$p(z)$}{probability distribution of $Z$}
\nomenclature[B, 20]{$P_1$, $P_2$}{two locations in wing--body juncture flow}
\nomenclature[B, 21]{$P$}{mean pressure}
\nomenclature[B, 21]{$\mathbb{P}$}{(discrete) probability mass function}
\nomenclature[B, 21]{$\mathsf{P}$}{covariance matrix of state vector}
\nomenclature[B, 21]{$\mathcal{P}$}{production (of TKE, Reynolds stresses, or turbulent frequency) }
\nomenclature[B, 24]{$\bm{q}$}{mean flow features}
\nomenclature[B, 25]{$Q^{\delta}$}{rotation matrix}
\nomenclature[B, 26]{$\mathsf{R}$}{covariance matrix of observation error}
\nomenclature[B, 26]{$\mathbb{R}$}{real number space}
\nomenclature[B, 27a]{$\bm{S}$}{strain rate tensor}
\nomenclature[B, 27b]{$\mathcal{S}$}{source terms}
\nomenclature[B, 27c]{${S}_i$}{scenario (in BMSA)}
\nomenclature[B, 27d]{$t$}{time}
\nomenclature[B, 27e]{$T_\omega$}{transport of turbulent frequency}
\nomenclature[B, 28]{$u_i$, $\bm{u}$}{instantaneous velocity}
\nomenclature[B, 29]{$u'_i$, $\bm{u}'$}{velocity fluctuation}
\nomenclature[B, 30]{$U_i$, $\bm{U}$}{mean velocity}
\nomenclature[B, 31]{$\mathbb{V}\text{ar}[Z]$}{variance of random variable $Z$}
\nomenclature[B, 32a]{$\mathbf{V}$}{eigenvectors of second order tensor}
\nomenclature[B, 32b]{$w_\alpha$ }{coefficients in expansion of random field}
\nomenclature[B, 32c]{$W$ }{Wiener process (in SDEs) }
\nomenclature[B, 33]{$x_i$, $\bm{x}$ }{spatial coordinate}
\nomenclature[B, 34]{$y$ }{model output}
\nomenclature[B, 36]{$z$}{model-predicted quantity}
\nomenclature[B, 35]{$Z$, $z$}{random variable and its realization}

\nomenclature[C, 01]{$\alpha$}{index for basis functions}
\nomenclature[C, 02]{$\beta$}{multiplicative discrepancy field}
\nomenclature[C, 03]{$\gamma$}{parameter in regularization term}
\nomenclature[C, 04a]{$\delta$}{discrepancies}
\nomenclature[C, 04b]{$\delta_{ij}$}{Kronecker delta, second-order identity tensor}
\nomenclature[C, 04]{$\Delta_g$}{grid spacing/filter width in LES}
\nomenclature[C, 05]{$\epsilon$}{noise in experimental data}
\nomenclature[C, 05]{$\varepsilon$}{dissipation rate}
\nomenclature[C, 06]{$\zeta$}{truth in the context of model uncertainty}
\nomenclature[C, 07]{$\theta$, $\bm{\theta}$}{model parameter(s)}
\nomenclature[C, 07]{$\vartheta$}{angle of rotation}
\nomenclature[C, 08]{$\kappa$}{von Karman constant}
\nomenclature[C, 09]{$\lambda_i$}{eigenvalues for anisotropy tensor}
\nomenclature[C, 09]{$\mathbf{\Lambda}$}{diagonal matrix of eigenvalues for anisotropy tensor}
\nomenclature[C, 10]{$\mu$}{dynamic viscosity of fluids}
\nomenclature[C, 11]{$\nu$}{kinematic viscosity}
\nomenclature[C, 11b]{$\nu_t$}{turbulent eddy viscosity}
\nomenclature[C, 12a]{$\xi$}{physical state of the system}
\nomenclature[C, 13]{$\rho$}{fluid density}
\nomenclature[C, 13b]{$\bm{\varsigma}$}{latent variables  (e.g., geometry, boundary conditions in CFD model)}
\nomenclature[C, 14a]{$\sigma$}{variance (field) of random fields}
\nomenclature[C, 14b]{$\sigma_k$, $\sigma_{\varepsilon}$}{coefficients in turbulence models}
\nomenclature[C, 14c]{$\Sigma$}{covariance matrix}
\nomenclature[C, 15]{$\bm{\tau}$}{Reynolds stress}
\nomenclature[C, 16]{$\nu_t$}{turbulent viscosity}
\nomenclature[C, 17]{$\phi_i(\bm{x})$}{basis functions (e.g., from Karhunen--Loeve expansion)}
\nomenclature[C, 18]{$\varphi_i$}{Euler angles}
\nomenclature[C, 19]{$\Psi$}{quantities of interest}
\nomenclature[C, 20]{$\omega$ }{turbulent frequency}
\nomenclature[C, 21]{$\mathbf{\Omega}$}{rotation-rate tensor}


\nomenclature[D, 00]{BMSA}{Bayesian model--scenario averaging}
\nomenclature[D, 01]{CFD}{computational fluid dynamics}
% \nomenclature[D, 02]{cdf}{ cumulative distribution function}
\nomenclature[D, 03]{DNS}{direct numerical simulation}
\nomenclature[D, 04]{EARSM}{explicit algebraic Reynolds stress model }
\nomenclature[D, 05]{EnKF}{ensemble Kalman filtering}
\nomenclature[D, 06]{gPC}{generalized  polynomial chaos }
\nomenclature[D, 07]{LES}{large eddy simulation}
\nomenclature[D, 07]{LHS}{Latin hypercube sampling}
\nomenclature[D, 08]{PCE}{polynomial chaos expansion}
\nomenclature[D, 09]{PDE}{partial differential equation}
\nomenclature[D, 10]{pdf}{ probability density function}
\nomenclature[D, 11]{pmf}{probability mass function}
\nomenclature[D, 12]{QoI}{quantity of interest}
\nomenclature[D, 13]{MCMC}{Markov chain Monte Carlo}
\nomenclature[D, 14]{NS}{Navier--Stokes}
\nomenclature[D, 15]{RANS}{Reynolds-averaged Navier--Stokes}
\nomenclature[D, 16a]{RSTE}{Reynolds stress transport equation}
\nomenclature[D, 16b]{RSTM}{Reynolds stress transport model}
\nomenclature[D, 16c]{SA}{Spalart--Allmaras (turbulence model)}
\nomenclature[D, 17]{SDE}{stochastic differential equation}
\nomenclature[D, 17]{SGS}{sub-grid scale}
\nomenclature[D, 18]{TKE}{turbulent kinetic energy}
\nomenclature[D, 18]{UQ}{uncertainty quantification}

\printnomenclature[1.1cm]

